Accountable Anonymous Group Messaging

Users often wish to participate in online groups anonymously, but misbehaving users may abuse this anonymity to spam or disrupt the group. Messaging protocols such as Mix-nets and DC-nets leave online groups vulnerable to denial-of-service and Sybil attacks, while accountable voting protocols are unusable or inefficient for general anonymous messaging. We present the first general messaging protocol that offers provable anonymity with accountability for moderate-size groups, and efficiently handles unbalanced loads where few members have much data to transmit in a given round. The N group members first cooperatively shuffle an NxN matrix of pseudorandom seeds, then use these seeds in N "pre-planned" DC-nets protocol runs. Each DC-nets run transmits the variable-length bulk data comprising one member's message, using the minimum number of bits required for anonymity under our attack model. The protocol preserves message integrity and one-to-one correspondence between members and messages, makes denial-of-service attacks by members traceable to the culprit, and efficiently handles large and unbalanced message loads. A working prototype demonstrates the protocol's practicality for anonymous messaging in groups of 40+ member nodes.

==> definitions.tex <==
\subsection{Definitions}

	\paragraph{Cryptographic Primitives}
	We make use of the standard (possibly randomized) \textit{signature scheme}
	defined as in Brickell and Shmatikov paper \cite{DBLP:conf/kdd/BrickellS06}.
	We will denote the signature of a message $m$ with key $u$
	as \sig{u}{m}.

	We adopt the definition of a \textit{public-key cryptosystem} from
	Fujisaki et al. \cite{Fujisaki:2004fk}.
	We modify this definition slightly, requiring that the
	randomness $r$ used to encrypt a message is recoverable
	during decryption.  We also require that the cryptosystem
	in use be IND-CCA2 secure \cite{bellare1998cryptodefs}.
	As in Justin Brickell and Vitaly Shmatikov's paper on
	anonymous data collection, we denote the encryption of
	message $m$ with public key $y$ as $\E{m}{y}$
	\cite{DBLP:conf/kdd/BrickellS06}.
	To denote the serial encryption of message $m$ with
	public keys $y_N, \ldots, y_1$, we will write
	$\E{m}{y_{N}:y_1}$.

	We use the standard definition \cite{Stinson} of an \textit{unkeyed
	hash function} and will denote the hash of message $m$ as
	$\hash{m}$.

	We use a standard definition \cite{Stinson} of a \textit{pseudo-random bit
	generator}.  We will denote the first $L$ bits generated from
	a pseudo-random bit generator seeded with $s$ as \rand{L}{s}.

	\begin{comment}
%%%%%%
	\paragraph{Signature Scheme}
		We use the definition of a signature scheme from Justin
		Brickell and Vitaly Shmatikov's anonymous
		data exchange protocol \cite{DBLP:conf/kdd/BrickellS06}.
		Brickell and Shmatikov define a digital signature scheme
		$(\mathcal{K}, \textsc{sig}, \mathcal{V})$ as consisting of
		three algorithms:
		\begin{itemize}
			\item 	The randomized \textit{key generation} algorithm
					$\mathcal{K}$ produces a private/public key pair
					$(u,v)$.
			\item 	The \textit{signing algorithm} \textsc{sig} takes
					a private key $u$ and produces a signature
					$\sigma = \textsc{sig}_u\{m\}$.
			\item 	The \textit{verification} algorithm $\mathcal{V}$
					takes a public key $v$, a message $m$, and a
					candidate signature $\sigma$.  $\mathcal{V}$ returns
					1 if $\sigma$ is a valid signature of $m$ with key
					$u$ and 0 otherwise.
					$\mathcal{V}(v, m, \textit{sig}_u\{m\})$ always
					returns 1.
		\end{itemize}
	
	\paragraph{Probabilistic Public-Key Cryptosystem}
		We use the definition for a probabilistic public-key
		cryptosystem from Fujisaki et al.'s investigation of
		the security of the OAEP cryptosystem \cite{Fujisaki:2004fk}.
		We modify this definition slightly, requiring that the
		randomness $r$ used to encrypt a message is recoverable
		during decryption.  We also require that the cryptosystem
		in use be IND-CCA2 secure \cite{bellare1998cryptodefs}.
		Notably, the Optimal
		Asymmetric Encryption family of cryptosystems (including
		RSA-OAEP) satisfies these requirements \cite{Bellare:1995fk}
		Fujisaki et al. define a public-key encryption scheme
		$(\mathcal{K}, \mathcal{E}, \mathcal{D})$
		over a message space $\mathcal{M}$ by three algorithms:
		\begin{itemize}
			\item 	The \textit{key-generation} algorithm
					$\mathcal{K}(1^\rho)$, where $\rho$ is the
					security parameter, produces a private/public
					key pair $(x,y)$.  Algorithm $\mathcal{K}$ is
					probabilistic.
			\item 	The \textit{encryption} algorithm
					$\mathcal{E}_y(m, r)$ outputs a ciphertext
					$c$ corresponding to the plaintext
					$m \in \mathcal{M}$ using randomness $r$.
			\item 	The \textit{decryption} algorithm
					$\mathcal{D}_x(c)$ outputs the plaintext $m$
					associated to the ciphertext $c$ and the
					randomness $r$ used to encrypt $m$.
		\end{itemize}
	
		As in Justin Brickell and Vitaly Shmatikov's paper on
		anonymous data collection, we denote the encryption of
		message $m$ with public key $y$ as $\E{m}{y}$
		\cite{DBLP:conf/kdd/BrickellS06}.
		To denote the serial encryption of message $m$ with
		public keys $y_N, \ldots, y_1$, we will write
		$\E{m}{y_{N}:y_1}$.
	
	\paragraph{Hash Function}
		We use the definition of a hash function from Douglas
		Stimpson's book on cryptographic theory \cite{Stinson}.
		An \textit{unkeyed hash function} is a function
		$h: \mathcal{X} \rightarrow \mathcal{Y}$ where $\mathcal{X}$
		is a set of possible messages and $\mathcal{Y}$ is a finite
		set of possible message digests.

		(XXX) What kind of crypto properties needed?

	\paragraph{Pseudo-random Number Generator}
		We use the definition of a bit generator from Douglas
		Stimpson's book on cryptographic theory \cite{Stinson}.
		A $(k,l)$-\textit{bit generator} is a function
		$f : (\mathbb{Z}_2)^k \rightarrow (\mathbb{Z}_2)^l$
		that can be computed in polynomial time (as a function
		of $k$) such that $l \geq k+1$.  The \textit{seed}
		is the input $s_0 \in (\mathbb{Z}_2)^k$ and the output
		$f(s_0) \in (\mathbb{Z}_2)^l$ is called the
		\textit{generated bitstring}.

		(XXX) What kind of crypto properties needed?
%%%%%%
	\end{comment}

	\paragraph{Honesty}
		A participant is \textit{honest} if she participant
		follows the protocol specification exactly.  
		Participants who stop sending messages during the protocol's
		execution may be doing so honestly (if the network connection
		failed, for example) or with the intention of disrupting
		the protocol (dishonestly).  The problem of how to distinguish
		between these two types of ``silent" participants is outside
		of the scope of this paper.  We refer interested readers to
		PeerReview for further discussion of this topic
		\cite{haeberlen07peerreview}.
		
	\paragraph{Integrity}
		The protocol maintains \textit{integrity}
		if, at the end of a run of the protocol, every honest
		participant either
		\begin{enumerate}
			\item 	Holds the plaintext of every other honest
					participant, or
			\item 	Knows that the plaintext of at least one
					honest participant  has been corrupted.
		\end{enumerate}
				
	\paragraph{Anonymity}
		We use Brickell and 
		Shmatikov's definition of
		anonymity \cite{DBLP:conf/kdd/BrickellS06}.  In a run
		of the protocol, a subset of dishonest participants may
		collude with the intent of matching the messages of honest
		participants to their authors.  We say that the
		protocol maintains \textit{collusion-resistant anonymity}
		if a group of $k$ colluding participants out of $N$ total
		participants (with $k \leq N-2$) cannot match an honest
		participant's message to the message's author with a
		probability better than random guessing.
	
		To formalize this definition, Brickell and Shmatikov define
		an ``anonymity game'' played between a challenger playing
		the role of the dishonest colluding participants and an
		oracle playing the role of the honest participants
		\cite{DBLP:conf/kdd/BrickellS06}.  Those interested in
		the specifics of the anonymity game should refer to
		the Brickell-Shmatikov paper.  The protocol
		maintains \textit{collusion-resistant anonymity} if, for
		all probabilistic polynomial-time challengers, the advantage
		in the anonymity game is negligible.
	
	\paragraph{Accountability}		
		We adopt the terminology from PeerReview to describe the
		notion of accountability \cite{haeberlen07peerreview}.  A
		participant $i$ is \textit{exposed} by participant $j$ if
		$j$ has a proof of $i$'s misbehavior.  
		The protocol maintains \textit{accountability} if, at the
		end of the protocol, either
		\begin{enumerate}
			\item 	All honest participants have the plaintexts
					of all honest participants, or
			\item 	At least one dishonest participant is exposed
					by all honest participants.
		\end{enumerate}
\com{
	\paragraph{Repudiability}
		We adopt the notion of repudiability from
		Borisov et al. \cite{borisov04offtherecord}.  The protocol maintains
		\textit{repudiability} if no participant can individually produce
		a proof that she did \textit{not} send a particular message.

		In other words, no participant can ``disown" an anonymously transmitted
		message after the protocol terminates.  
}


==> future.tex <==
\section{Further Extensions}

(possibly to be merely summarized or left for future work)

\begin{itemize}
\item	Content accountability:
	Suppose it is desired for the group of participants
	to be able to evaluate each anonymously broadcast message
	and collectively decide whether or not the anonymity
	of that message's sender should be preserved:
	e.g., based on whether or not the content broadcast
	was ``legal'' or ``responsible'' according to group consensus.
	The protocol can be easily modified
	to provide this form of accountability as follows:
	\begin{enumerate}
	\item	Change the dining cryptographers extension
		so that of all the messages ``proposed'' in the first phase,
		only the owner of the {\em first} transmission slot
		with some message to transmit ($L > 0$)
		actually transmits in the second, dining cryptographers phase.
		The first phase now essentially implements
		a randomized arbiter for exclusive use of
		the second phase message channel;
		if multiple participants wish to send messages,
		the others must do so in later, independent protocol runs.
		All participants for now retain the ``blame'' information
		they would have used in the first phase
		to trace a dishonest DoS attacker,
		even if the first and second phases succeed.

	\item	Once all the participants obtain
		the anonymously transmitted message,
		they evaluate it and decide by some collective process,
		such as a vote,
		whether to preserve or unmask the message sender's identity.
		The participants can perform an integrity-protected vote,
		for example,
		simply by rerunning the first phase algorithm
		with ballots as the anonymously published messages.
		If some agreed-upon threshold or quorum of participants
		votes to unmask the sender,
		then all honest nodes release their blame information.
		This process will expose either the sender
		{\em or} some dishonest node:
		i.e., any dishonest node can choose to ``take the fall''
		for the actual message sender,
		but presumably that's OK.
	\end{enumerate}

\item	Further efficiency enhancements:
	The following refinement should reduce
	the message complexity of the dining cryptographers extension
	from $O(N^3 + log L_{max} N^2 + L_{total} N)$
	to $O(N^2 + L_{total} N)$,
	and simultaneously enable the participants
	to repeat the dining cryptographers phase any number of times
	with newly chosen messages
	after only one run of the first shuffle phase,
	thereby amortizing the $O(N^2)$ shuffle cost
	over many subsequent messages.
	In this protocol variant,
	each participant uses the shuffle phase to publish
	a public key usable for Diffie-Hellman key exchange
	to all other participants,
	allowing each participant to form a shared secret
	with all other participants without knowing
	which actual participant holds each of the other public keys.

	From each of these $N^2$ shared ``master secrets,''
	the participants generate two derived shared secrets:
	a seed for an ordinary pseudorandom function,
	and a simulable, verifiable random function (sVRF).
	The secrets shared between {\em different} participants
	($i \ne j$) yield true VRFs from the sVRF's function space,
	and the degenerate secrets for $i = j$ cases
	yield simulated VRFs controlled by the owner participant.

	Each participant $i$ now creates a commitment message, containing:
	(1) a list of participant $i$'s $N$ sVRF public keys,
	in anonymous transmission slot order order, and
	(2) a list of hashes of participant $i$'s $N$ shared master secrets,
	in random order.
	Participant $i$ sends its signed commit message to participant 1,
	which collects all the commit messages, hashes each,
	and broadcasts a list of the resulting $N$ hashes,
	in order of participant number, to all participants.
	Each participant verifies that its correct hash
	appears in the correct slot,
	and participants broadcast GO/NO-GO messages
	(which may be combined with the GO/NO-GO messages
	required by the regular shuffle protocol's verification phase).

	The participants then engage in
	any number of message transmission rounds,
	via the following variant of the dining cryptographers extension.
	First, the participants transmit small fixed-length messages
	indicating the lengths of the actual messages they wish to transmit,
	using the regular shared pseudo-random number seeds
	to generate the ``anonymity cloak'' for each transmission slot.
	Second, the participants transmit the content of the actual messages,
	again using the regular pseudo-random number seeds
	to maintain anonymity.
	Third, each participant transmits anonymously,
	this time using the set of sVRFs for its anonymous transmission slot,
	a small, fixed-length {\em validation} or {\em accusation}.
	If participant $i$ is satisfied
	with the results of the anonymous transmission of its slot,
	then $i$ transmits a {\em validation} containing a hash
	of the length and content of the message it transmitted.
	If participant $i$ detects
	that another participant corrupted its message, however,
	then $i$ transmits an {\em accusation}
	containing the accused participant number $j$
	and the master secret shared between $i$ and $j$.

	When the participants see a validation appear with the correct hash
	in a given anonymous transmission slot,
	they can be confident of the integrity of the message in that slot
	provided the sender is honest,
	because the value the honest sender XORs into the validation slot
	is not known or predictable by any dishonest nodes,
	and thus dishonest nodes cannot cause a correct validation to appear
	for a forged message with non-negligible probability.

	When the participants see anything other than
	a correct validation of the correct message/length hash,
	they first check the XORed components of the validation/accusation
	against all of the sVRF public keys for that slot
	(retrieving those public keys from participant 1 if necessary).
	Any failures at this stage
	expose the generating participant(s) as dishonest,
	without revealing any information about which sVRF
	corresponded to the transmitter for that slot
	(i.e., the participant holding the simulated VRF
	rather than one of the $N-1$ true VRFs from the sVRF's function space).
	If an accusation passes this sVRF check,
	then the participants verify the shared master secret
	revealed by the accusation
	against the master secret hashes
	in the participants' original commit messages,
	and check the pseudorandom stream generated by the accused participant
	during anonymous message transmission
	against the bits the participant should have generated
	from its master secret.
	If the accusation checks out,
	then the accused participant is exposed as dishonest.

	If the validation/accusation is corrupt or does not check out,
	then the participants know
	that the anonymous sender for that slot is itself at fault.
	The participants {\em could} then unmask the identity
	of the faulty sender,
	by revealing all of their secrets shared with that transmission slot.
	In practice, however, such drastic action may not be desirable because
	(a) the faulty sender has only corrupted its own message transmission,
	and not that of any other node, causing no permanent harm; and
	(b) if the sender somehow became faulty {\em after}
	some number of successful message rounds
	during which the sender was correct and honest,
	then unmasking the sender's identity would unnecessarily
	compromise the anonymity of {\em all} of its transmissions
	including those it transmitted before it became faulty.
	As one alternative, therefore,
	the participants could merely
	eliminate the faulty participant's transmission slot
	from all future transmission rounds,
	thereby preventing the faulty sender from wasting
	the group's time and bandwidth while preserving its anonymity.
	(If the faulty sender does not ``bow out gracefully''
	according to this protocol,
	it will corrupt subsequent transmissions and be exposed publicly.)
\end{itemize}



==> init.tex <==
\section{Protocol Initiation}
\label{sec:init}

The core protocols described above
assume that the set of nodes participating in a particular round
is already agreed-upon...

alternatives: round-robin leader, or consensus (e.g., BFT).
round-robin doesn't guarantee anything about consistency, ordering,
or whether multiple protocol instances can run at once.
BFT fixes that, with the disadavantage of making the group unavailable
any time two thirds or more of the members are faulty or dishonest.

also, problem of nodes that just stop communicating,
or communicate with some nodes but not others.

leader determines which nodes are alive and which are not,
decides the set of participating members for a given protocol instance...
A node is live iff leader considers it live.
If two non-leader nodes can communicate with the leader but not each other,
then we assume the leader can forward their traffic to each other,
thereby ensuring the desired connectivity invariant.

As in PeerReview: if the protocol calls for a particular member
to send a particular type of message at a particular stage,
any member needing that message can place the member under suspicion...
Leader decides when to time-out, consider the suspect member failed,
and restart the protocol without that member.

Efficiency issue:
a colluding group of $M$ malicious members
can prevent the group from making progress for $MT$ time,
where $T$ is the leader's progress timeout.
There is no way to prevent this when the malicious members are colluding,
since it is trivial for them to arrange for all but one colluding member
to behave honestly during each round,
so that the leader can identify and remove only one member per round.



==> keying.tex <==
\section{Deniable Keying}

The core protocols above require each participating member
to have a signing key pair whose public key is known to all other members,
and relies on the non-repudiability of messages signed with this key
to allow members to trace and provide proof of misbehavior
to the leader or other members.
Unfortunately, the non-repudiability of these signed messages
potentially leaves members vulnerable to coercion.

Suppose for example that a group of whistleblowing journals
leaks a document sensitive to a powerful government,
and the government in response places all the member journalists
in its jourisdiction under pressure
to prove that they were not the source of the leak.
If an otherwise-honest member saves all the information it used
while participating in a given protocol round,
rather than erasing it as the protocol requires---%
in particular, the randomness the member used for its public key encryptions
during phase 2 of the shuffle protocol---%
then the member can prove to the adversary beyond much doubt
which message the member was responsible for in that particular round,
simply by revealing that information.
If a member journalist feels he is likely to come under such pressure
after a given document is leaked,
and he is not the source of the leaked document,
that foresight might by itself give him a strong incentive
to save the secret information he used in the protocol
in case he needs to prove his innocence,
thereby placing himself in the ``dishonest'' camp
and reducing the anonymity of the true source of the document.
Worse, a member journalist who is given a sensitive document to be leaked,
but is under the jourisdiction of the affected government,
may feel reluctant to leak the document at all
despite the anonymity provided by the protocol,
out of fear he will be ``presumed guilty''
unless he can prove his innocence once he comes under pressure.

If the powerful adversary monitors all of the group's network traffic,
{\em and} the adversary's raw traffic logs are usable as evidence
to incriminate or acquit a member
once he has revealed his shuffle protocol secrets under pressure,
then there is nothing we can do at the protocol level
to reduce the member's vulnerability to coercion.
The member effectively ceases to be able to act independently of the adversary
if he can be forced to reveal all secrets
pertaining to any network traffic he produces.
If on the other hand the adversary is not omniscient in its traffic monitoring,
{\em or} its traffic logs alone are not sufficient evidence
to prove that a given network message was sent by a given member,
then we can increase the anonymity protocol's resistance to coercion
by making anonymity protocol exchanges {\em deniable}.
In particular, we wish to design the protocol
so that after a particular protocol run,
the messages produced in that run cannot be tied conclusively
to any of the participating members.
Ideally, we would like it to be the case
that {\em anyone} can unilaterally fabricate the entire set of messages
produced by any legitimate protocol run,
so that any member participating in a group
can later make a justifiable claim
that all the messages attributed to him
were in fact sent or fabricated by someone else.

\subsection{Deniable Signing Key Exchange}

Most existing deniable protocols
focus on generating authenticated shared secrets
for pairwise communication~\cite{XXX}.
Some work has been done on deniable group authentication~\cite{bohli06deniable},
but still with the goal of agreeing on a shared secret
for private communication.
For our purposes, however, a shared secret alone is not sufficient,
because our shuffle and bulk protocols require messages to be non-repudiable
at least {\em within a given protocol run},
so that misbehaving members can be traced and excluded.
Our solution to this dilemma
is to dissociate the signing keys members use in the shuffle and bulk protocols
from their long-term identities,
so that group members know these associations {\em during} the protocol run
but no one can prove them {\em after} the protocol completes.
Thus, each group member will generate a fresh signing key
for each protocol run,
and the group must use a deniable group authenticated protocol
to agree on the set of signing keys for a particular run
and their associations with long-term identities.
Since no existing group authentication protocol we are aware of
provides the necessary combination of properties,
we suggest the following protocol.

\begin{enumerate}
\item	Each member $i$ generates
	a temporary signing key pair ($u_i,v_i$) for this protocol run.

\item	Leader chooses a nonce $n_r$ identifying the protocol run,
	and a challenge nonce $c_{0,i}$ for each member $1 \le i \le N$,
	encrypts each $c_{0,i}$ with member $i$'s long-term public key $id_i$,
	and sends $n_r,\{c_{0,i}\}_{id_i}$ to member $i$.

\item	Upon receiving the leader's challenge message,
	member $i$ decrypts the nonce $n_r$ and challenge $c_{0,i}$.
	Member $i$ now chooses a random challenge $c_{i,j}$  % = H(n_r,v_i,i,j)$
	for each member $1 \le j \le N$,
	to permit $i$ to verify $j$'s identity.
	Member $i$ encrypts each $c_{i,j}$ with member $j$'s public key $id_j$,
	builds a response $R=n_r,\{v_i\}_{id_0},c_{i,1},\dots,c_{i,N}$,
	where $id_0$ is the leader's long-term public key,
	and sends $R,H_{c_{0,i}}(R)$ back to the leader.
	(If the leader is one of the participants,
	$id_0$ may be the same as one of the $id_i$ for $1 \le i \le N$).
	The hash keyed on $c_{0,i}$ authenticates this response to the leader,
	convincing the leader that $v_i$
	is $i$'s public signing key for this round
	and that the set of encrypted challenges were generated by member $i$.

\item	For each node $j$,
	the leader now collects the challenges $c_{i,j}$ from each node $i$
	into a list and sends $n_r,v_0,\dots,v_j,c_{0,j},\dots,c_{N,j}$
	to node $j$.  (XXX authenticate this message)

\item	Member $j$ receives the list of public keys and challenges,
	decrypts each challenge $c_{i,j}$ with its private key,
	and returns a response $H_{c_{i,j}}(n_r,j,v_j)$
	to member $i$ via the leader,
	convincing member $i$ that $v_j$ is indeed $j$'s public key
	for this round.

\item	If any of the ``peer-to-peer'' challenges fails to match,
	then the challenging node complains
	and the leader enters a blame phase to determine
	which member is faulty.
	In such a dispute, the challenging node $i$
	must prove its innocence to the leader by revealing
	the randomness it used to encrypt its challenge to node $j$.
	The leader can then replay that encryption
	and check it against the challengee's response
	to determine whether the challenger or challengee was at fault,
	and start a new protocol run with the faulty node excluded.
\end{enumerate}

In a particular protocol run,
if the leader is faulty,
we can of course make no statements about the protocol making progress:
instead, we rely on some other non-faulty member
subsequently taking the leadership role,
either by a simple schedule or by byzantine agreement
as discussed earlier in Section~\ref{sec:init} (XXX),
so that progress may be guaranteed in a later protocol run.

XXX The above can be simplified
if we just state that the leader first
forms a pairwise communication channel with each other member
using standard deniable authenticated key exchange~\cite{raimondo05secure},
and obtains a master list of public keys for the new round that way,
so the above protocol {\em only} has to worry about
authenticating members to each other against the leader's master list.



==> problem.tex <==
\subsection{Problem Statement}

	A run of the protocol involves a group of $N$ members who
	may be unreliable or dishonest.  Each group member has a well-known
	long-term public-key encryption keypair, a signing keypair, 
	and a message of arbitrary length (up to some maximum length).
	We assume that group members have labeled themselves $1, \ldots, N$
	and that the group collectively maintains a session 
	counter.  (In practice, the group could agree upon the ordering
	and session counter using the Paxos protocol \cite{Lamport:1998}.)

	After executing the protocol, every honest group member
	should hold the messages of all other honest group members.
	Additionally, we require that the protocol maintain
	\textit{integrity}, \textit{anonymity}, and \textit{accountability}
	even when confronted with a polynomial-time adversary who can
	eavesdrop on all network traffic.

	\com{
	For our purposes, breaking the anonymity of the protocol requires only that the
	adversary ``prove'' to herself that a group member authored a particular
	message.  In particular, the adversary's traffic logs are sufficient to
	prove that a group member send a certain message.
	This assumption is reasonable for practical situations, where the adversary
	might be the secret police of a totalitarian government.  The secret police
	need not formally prove to anyone but itself that a member authored a
	message but only needs to convince itself of the fact.

	If traffic logs are not a sufficient proof of authorship of a particular message,
	then there exist other schemes that provide anonymous message signature schemes
	that do not provide protection against network traffic analysis \cite{Rivest:2001}.

	The group must also have some method for dealing with members
	who stop responding during a run of the protocol.  Since group members might
	stop communicating for legitimate reasons (e.g. a network failure) or 
	for nefarious reasons (e.g. to execute a DoS attack), the group must have
	some method of coping with this type of fault.  Addressing this ``silent node''
	issue is outside of the scope of this paper, but practical systems do exist to 
	cope with it \cite{haeberlen07peerreview}.
	}




==> todo.tex <==
\section{Still to do}
	\begin{itemize}
		\item Change ``participant'' to ``member'' everywhere?
		\item Establish crypto properties we want for Hash, PRNG

	\end{itemize}

